Curriculum Design for Teaching via Demonstrations: Theory and Applications

We consider the problem of teaching via demonstrations in sequential decision-making settings. In particular, we study how to design a personalized curriculum over demonstrations to speed up the learner's convergence. We provide a unified curriculum strategy for two popular learner models: Maximum Causal Entropy Inverse Reinforcement Learning (MaxEnt-IRL) and Cross-Entropy Behavioral Cloning (CrossEnt-BC). Our unified strategy induces a ranking over demonstrations based on a notion of difficulty scores computed w.r.t. the teacher's optimal policy and the learner's current policy. Compared to the state of the art, our strategy doesn't require access to the learner's internal dynamics and still enjoys similar convergence guarantees under mild technical conditions. Furthermore, we adapt our curriculum strategy to the setting where no teacher agent is present using task-specific difficulty scores. Experiments on a synthetic car driving environment and navigation-based environments demonstrate the effectiveness of our curriculum strategy.

==> checklist.tex <==
\clearpage
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \looseness-1\answerYes{In Sections \ref{sec:curr-teacher-algo} and \ref{sec:curr-teacher-theory}, we present our curriculum strategy and provide theoretical analysis as described in the introduction. The experimental results mentioned in the abstract and introduction are detailed in Sections \ref{sec:experiments} and \ref{sec:experiment_without_teacher}.}
  \item Did you describe the limitations of your work?
    \answerYes{We discuss the limitations of our work in Sections \ref{sec:experiments} and \ref{sec:conclusion}. We point out that convergence bounds for \bcmodel~learners have not been obtained yet and that it would be beneficial to explore approaches to estimate the learner's policy $\pi^L_t$ using fewer queries.
    % Both of these would be interesting directions for future work.
    }
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{As stated in Section \ref{sec:conclusion}, this work presents the theoretical underpinnings of curriculum design for teaching via demonstrations. This can be beneficial for education applications and for self-curriculum design for imitation learners. As such in the present form, we do not see any direct negative societal impacts of our work.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{We confirm that our paper conforms with the ethics review guidelines.}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{In Section \ref{subsec:max-ent}, we state our assumptions of a deterministic MDP and linear reward structure. Similarly, we state our assumption of a linear scoring function for the \bcmodel~learner in Section \ref{subsec:cross-ent}. The simplifications considered are reiterated in the proofs.}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{Complete proofs of all theoretical results are included in the Appendix.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{The code and instructions are included as a URL.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Training details are presented in the Appendix and are also present in the code.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{Error bars are included in all the result graphs, as can be seen in figures.}
    % \ref{fig:IRL.reward_and_curriculum}, \ref{fig:BC.expected.reward} and \ref{fig:wsp_results}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{The details are provided in the Appendix.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerNA{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
